Restrictions on Weil polynomials of Jacobians of hyperelliptic curves

Inspired by experimental data, this paper investigates which isogeny classes of abelian varieties defined over a finite field of odd characteristic contain the Jacobian of a hyperelliptic curve. We provide a necessary condition by demonstrating that the Weil polynomial of a hyperelliptic Jacobian must have a particular form modulo 2. For fixed ${g\geq1}$, the proportion of isogeny classes of $g$ dimensional abelian varieties defined over $\mathbb{F}_q$ which fail this condition is $1 - Q(2g + 2)/2^g$ as $q\to\infty$ ranges over odd prime powers, where $Q(n)$ denotes the number of partitions of $n$ into odd parts.

==> genus3_table.tex <==
\begin{tabular}{l|cc|r}
$q$
&
No hyperelliptic Jacobian
&
Ruled out by Thm.~\ref{main-thm-g3}
&
Total
\\
\hline
\multirow{2}{*}{\numprint{3}}
&
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=3&hyp_cnt=0}{\numprint{380}}
&
\numprint{168}
&
\numprint{677}
\\
&
56.13\%
&
24.82\%
\\
\multirow{2}{*}{\numprint{5}}
&
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=5&hyp_cnt=0}{\numprint{1230}} &
\numprint{716}
&
\numprint{2953}
\\
&
41.65\%
&
24.25\%
\\
\multirow{2}{*}{\numprint{7}}
&
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=0}{\numprint{2748}} &
\numprint{1984}
&
\numprint{7979}
\\
&
34.44\%
&
24.87\%
\\
\multirow{2}{*}{\numprint{9}}
&
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=0}{\numprint{5830}}
&
\numprint{3732}
&
\numprint{15459}
\\
&
37.71\%
&
24.14\%
\\
\multirow{2}{*}{\numprint{11}}
&
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=0}{\numprint{8842}}
&
\numprint{7564}
&
\numprint{30543}
\\
&
28.95\%
&
24.77\%
\\
\multirow{2}{*}{\numprint{13}}
&
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=0}{\numprint{13997}}
         &
\numprint{12544}
&
\numprint{50371}
\\
&
27.39\%
&
24.90\%
\end{tabular}


==> hyp_count_table.tex <==
\begin{tabular}{l|cccccc|r}
  \multirow{2}{*}{$q$}& \multicolumn{6}{c|}{Number of hyperelliptic Jacobians} & \multirow{2}{*}{Total}\\
&
0 &
1 &
2 &
3-8 &
9-32 &
33-6375 &
\\
\hline
\multirow{2}{*}{\numprint{2}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=2&hyp_cnt=0}{\numprint{156}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=2&hyp_cnt=1}{\numprint{44}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=2&hyp_cnt=2}{\numprint{13}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=2&hyp_cnt=3-8}{\numprint{2}} &
 &
 &
215
\\
 &
72.56\% &
20.47\% &
6.05\% &
0.93\% &
 &
 &

\\
\multirow{2}{*}{\numprint{3}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=3&hyp_cnt=0}{\numprint{380}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=3&hyp_cnt=1}{\numprint{166}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=3&hyp_cnt=2}{\numprint{76}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=3&hyp_cnt=3-8}{\numprint{55}} &
 &
 &
677
\\
 &
56.13\% &
24.52\% &
11.23\% &
8.12\% &
 &
 &

\\
\multirow{2}{*}{\numprint{5}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=5&hyp_cnt=0}{\numprint{1230}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=5&hyp_cnt=1}{\numprint{438}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=5&hyp_cnt=2}{\numprint{374}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=5&hyp_cnt=3-8}{\numprint{767}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=5&hyp_cnt=9-32}{\numprint{144}} &
 &
2953
\\
 &
41.65\% &
14.83\% &
12.67\% &
25.97\% &
4.88\% &
 &

\\
\multirow{2}{*}{\numprint{7}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=0}{\numprint{2748}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=1}{\numprint{705}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=2}{\numprint{723}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=3-8}{\numprint{2531}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=9-32}{\numprint{1208}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=7&hyp_cnt=33-6375}{\numprint{64}} &
7979
\\
 &
34.44\% &
8.84\% &
9.06\% &
31.72\% &
15.14\% &
0.80\% &

\\
\multirow{2}{*}{\numprint{9}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=0}{\numprint{5830}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=1}{\numprint{56}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=2}{\numprint{1662}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=3-8}{\numprint{3510}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=9-32}{\numprint{3773}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=9&hyp_cnt=33-6375}{\numprint{628}} &
15459
\\
 &
37.71\% &
0.36\% &
10.75\% &
22.71\% &
24.41\% &
4.06\% &

\\
\multirow{2}{*}{\numprint{11}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=0}{\numprint{8842}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=1}{\numprint{1056}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=2}{\numprint{1122}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=3-8}{\numprint{7281}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=9-32}{\numprint{10153}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=11&hyp_cnt=33-6375}{\numprint{2089}} &
30543
\\
 &
28.95\% &
3.46\% &
3.67\% &
23.84\% &
33.24\% &
6.84\% &

\\
\multirow{2}{*}{\numprint{13}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=0}{\numprint{13997}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=1}{\numprint{1204}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=2}{\numprint{1324}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=3-8}{\numprint{8815}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=9-32}{\numprint{18805}} &
\href{https://www.lmfdb.org/Variety/Abelian/Fq/?g=3&q=13&hyp_cnt=33-6375}{\numprint{6226}} &
50371
\\
 &
27.79\% &
2.39\% &
2.63\% &
17.50\% &
37.33\% &
12.36\% &
\end{tabular}

